Can We Trust AI-Generated Educational Content? Comparative Analysis of Human and AI-Generated Learning Resources

As an increasing number of students move to online learning platforms that deliver personalized learning experiences, there is a great need for the production of high-quality educational content. Large language models (LLMs) appear to offer a promising solution to the rapid creation of learning materials at scale, reducing the burden on instructors. In this study, we investigated the potential for LLMs to produce learning resources in an introductory programming context, by comparing the quality of the resources generated by an LLM with those created by students as part of a learnersourcing activity. Using a blind evaluation, students rated the correctness and helpfulness of resources generated by AI and their peers, after both were initially provided with identical exemplars. Our results show that the quality of AI-generated resources, as perceived by students, is equivalent to the quality of resources generated by their peers. This suggests that AI-generated resources may serve as viable supplementary material in certain contexts. Resources generated by LLMs tend to closely mirror the given exemplars, whereas student-generated resources exhibit greater variety in terms of content length and specific syntax features used. The study highlights the need for further research exploring different types of learning resources and a broader range of subject areas, and understanding the long-term impact of AI-generated resources on learning outcomes.

==> article-highlights.tex <==
\begin{highlights}
\item The paper presents a unique comparison of student-generated and AI-generated creation of code examples using identical priming examples given by instructors. 
%\item The comparison is based on the overall length, syntax features, and perceived correctness and helpfulness of the resources.
\item Results suggest that AI-generated code closely aligns with instructors' examples, whereas student outputs demonstrate more autonomy and exhibit a greater range of styles and lengths.
\item Results also demonstrate a comparable perceived quality in terms of both correctness and helpfulness.
\item add one point on implications?
\end{highlights}

